Continuous rational functions are deterministic regular

A word-to-word function is rational if it can be realized by a non-deterministic one-way transducer. Over finite words, it is a classical result that any rational function is regular, i.e. it can be computed by a deterministic two-way transducer, or equivalently, by a deterministic streaming string transducer (a one-way automaton which manipulates string registers). This result no longer holds for infinite words, since a non-deterministic one-way transducer can guess, and check along its run, properties such as infinitely many occurrences of some pattern, which is impossible for a deterministic machine. In this paper, we identify the class of rational functions over infinite words which are also computable by a deterministic two-way transducer. It coincides with the class of rational functions which are continuous, and this property can thus be decided. This solves an open question raised in a previous paper of Dave et al.

==> parts/poubelle.tex <==

\begin{lemma}
\label{lem:pref}
Let $p_1, \dots, p_k \in I$,
$q_1, \dots, q_k \in Q$ be compatible,
$u \in A^*$, $v_1, \dots, v_k \in B^*$ be 
such that $p_i \xrightarrow{u| v_i} q_i$.
Then $\exists v\in A^*$ such that
$\forall 1 \le i \le k$, $v_i \pref v$.
\end{lemma}

\begin{proof}
Since $q_1, \dots, q_k$ are compatible,
there exists $x \in A^\omega$,
$y_1, \dots, y_k \in B^\omega$
such that for all $1 \le i \le k$, there exists a run.
$q_i \xrightarrow{x | y_i}$. Furthermore one of these runs
is accepting, suppose up to permutation that it is $q_1 \xrightarrow{x | y_1}$.
Hence $p_1 \xrightarrow{u| v_1} q_1  \xrightarrow{x | y_1}$ is a valid
run and $ux \in \dom{f}$.
Let $n \defined \max_i |v_i|$. Since $f$ is continuous in $ux$, there exists
$p \ge 0$ such that if $z \in \dom{f}$ and $|z \wedge ux| \ge p$,
then $|f(z) \wedge f(ux)| \ge n$. Since the transducer is
trim, for all $1 \le i \le k$, $\exists x_i \in A^\omega$ such
that $p_i \xrightarrow{u | v_i} q_i  \xrightarrow{x[1{:}p] | w_i} q'_i  \xrightarrow{x'_i | y'_i}$
is a valid run. Thus $f(u(x[1{:}p])x'_i) = v_i w_i y'_i$,
and finally $v_i \pref (f(ux))[1{:}n]$  for all $1 \le i \le k$.
\end{proof}







\begin{lemma}
Let $p_1, \dots, p_k \in I$,
$q_1, \dots, q_k \in Q$ be compatible.
Assume that there exists $u \in A^*$
and $\alpha_1, \dots, \alpha_k \in B^*$ $K$-remote
such that $p_i \xrightarrow{u| \alpha_i} q_i$.
Then there exists $\theta, \theta_1, \dots, \theta_k,\in B^*$ such that
the following holds.
If $v \in A^*$, $\beta_1, \dots, \beta_k \in B^*$,
$r_1, \dots, r_k \in Q$ are compatible and 
$q_i \xrightarrow{v| \beta_i} r_i$ for all $1 \le i \le k$, 
then $\beta_i  \pref \theta_i \theta^\omega$ for all $1 \le i \le k$.
\end{lemma}


\begin{proof} Assume up to permuting the $1 \le i \le k$ that $|\alpha_{1}| >  |\alpha_{2}| + K$.

\begin{claim} There exists $p'_1, \dots, p'_k \in Q$ and factorizations
$u = u'u''u'''$, $\alpha_i = \alpha'_i \alpha''_i \alpha'''_i$
such that $|\alpha''_1| > |\alpha''_2|$ and
forall $1 \le i \le k$,
$p_i \xrightarrow{u' | \alpha'_i} p'_i \xrightarrow{u'' | \alpha''_i}
p'_i \xrightarrow{u''' | \alpha'''_i} q_i$ is a run.
\end{claim}

\begin{iproof} \gd{Since} 

\end{iproof}
Since $r_1, \dots, r_k$ are compatible, Lemma~\ref{lem:compat} gives for all $1 \le i \le k$ a run:
\begin{equation*}
p_i \xrightarrow{u' | \alpha'_i} p'_i \xrightarrow{u'' | \alpha''_i}
p'_i \xrightarrow{u''' | \alpha'''_i} q_i
\xrightarrow{v| \beta_i} r_i  \xrightarrow{w|\gamma_i} r'_i\xrightarrow{w'| \gamma'_i} r'_i.
\end{equation*}
Furthermore there exists $1 \le j \le k$
such that $r'_j$ is accepting. Thus $\gamma'_j \neq \vide$.
Let us fix $m \ge 0$. Since $r'_1, \dots, r'_k$ are compatible,
by Lemma~\ref{lem:pref} for all $n \ge 0$
the $\alpha'_i (\alpha''_i)^m \alpha'''_i \beta_i \gamma_i (\gamma'_i)^n$
are prefixes of the same word. 
Since $\gamma'_j \neq \vide$, we get $\forall 1 \le i \le k$:
\begin{equation*}
\alpha'_i (\alpha''_i)^m \alpha'''_i \beta_i \gamma_i (\gamma'_i)^n
\pref \alpha'_j (\alpha''_j)^m \alpha'''_j \beta_j \gamma_j (\gamma'_j)^\omega.
\end{equation*}
If $m \ge |\alpha'''_i \beta_i \gamma_i|$


\end{proof}



















\subparagraph*{Conventions for multisets.} In the 
sequel we shall use \emph{multisets}, i.e. sets with repetitions
of elements. Given a finite set $X$, we denote by $\Mul(X)$ the set of multisets
over $X$. We denote by $\multi{x_1, x_2, \dots}$ the multiset
containing $x_1, x_2, \dots$. This notation allows repetitions,
i.e. we may equalities in the $x_i$. Similarly,
if $\mul \in \Mul(X) $, then  $ \mul = \multi{x \in \mul}$.
For $\mul \in \Mul(X)$, we denote by $|\mul|$ its \emph{size}, that is its number of elements including
repetitions. For instance $|\multi{x,x}| = 2$. Given $K \ge 0$, we denote by $\Mul^K(X) \subseteq \Mul(X)$ the set 
of multisets of size at most $K$. Note that the set $\Mul^K(X)$ is finite.



\begin{definition} Given a function $g:X \rightarrow Y$ and $K \ge 0$,
we extend it to a function on multisets $g : \Mul^{K}(X) \rightarrow \Mul^{K}(Y)$
by defining: $g(\mul) \defined \multi{g(x) : x \in \mul}$.
\end{definition}

\begin{remark}
Applying such an extension preserves the size, i.e.  $|\mul|  = |g(\mul)|$.
More  is in
fact a \emph{multiset bijection} between $\mul$ and $\mul$
\end{remark}

We shall also consider functions $g : \Mul^{K}(X)  \rightarrow Y$,
which are defined on a multiset. In this case, we consider
that the repetitions of the same element may have
different images (i.e. the function is not an extension
of a function defined on $X$).




\begin{lemma}
Let $u \in A^*$, $S \defined \cro{u}(I)$
and $x \in A^\omega$ such that $ux \in \dom{f}$,
There exists $C \subseteq S$ such that
 $C \in \Comp$  and $ \exists i \ge 0$ that $\cro{x[1{:}i]}(C) = \cro{x[1{:}i]}(S)$.
\end{lemma}

\begin{proof} Assume by contradiction that the property
of Lemma~\ref{lem:compat-fini} does not
hold. Let $P$ be the set of subsets $C = \{q_1, \dots, q_n\} \subseteq S$ 
such that:
\begin{itemize}
\item for all $1 \le i \le n$, there exists a run $\rho_i$
starting in $q_i$ and labelled by $x$;
\item $\exists 1 \le i \le n$ such that $\rho_i$ is accepting.
\end{itemize}
Then $P \subseteq \Comp$. Furthermore, $P$ is not empty.
Indeed,  since $ux \in \dom{f}$ there exists $q_1 \in S$ with a run $\rho_1$ which starts in $q_1$,
is labelled by $x$ and is accepting. Thus $\{q_1\} \in P$.

Now let us consider a set $C \in P$ such that
$|C| = \max_{C' \in P} |C'|$ (such a set exists).
Since $C \in \Comp$, then $\forall i \ge 0$ we must have
$\cro{x[1{:}i]}(C) \neq \cro{x[1{:}i]}(S)$,
thus $\cro{x[1{:}i]}(S \smallsetminus C) \neq \varnothing$
(because $\cro{x[1{:}i]}(S) = \cro{x[1{:}i]}(C) \cup \cro{x[1{:}i]}(S \smallsetminus C)$).
Hence the forest of all runs starting from $S \smallsetminus C$
and labelled by $x$ is infinite, thus by Kruskal's lemma it has
a infinite branch, i.e. there exists a state $q \in S \smallsetminus C$
and a run $\rho_q$ starting in $q$ and labelled by $x$.
Finally $C \uplus \{q\} \in P$, which contradicts
the maximality of $|C|$.
\end{proof}




\subparagraph*{Additional restrictions on the
transitions.} If $x \in \dom{f}$, we want to the unique
valid run to make the ``good'' choices, which is formalized
in Lemma~\ref{lem:unique-run} below. Before
its proof we shall describe the additional
restrictions on the transitions of $\mc{A}$
that make it become true.

In the description of the transitions on page~\pageref{p:trans},
we add the following conditions:
\begin{enumerate}
\item \gd{for all $(g,D) \in \Hist$, if $g(\reach) \neq \vide$ then $D \in g(\reach)$
(this will mean that if the set of accessible states is covered at some
point by the future of some compatible set, then the future of the chosen
compatible set covers it);}
\item \label{condi:un} for all $(g',C',D') \in \Hist'$, if $g'(D') = \vide$ and $g(D) \neq \vide$,
then $C'$ is the minimal element for $\pc$ in $g(D)$ (this will mean that
if the set of states reachable from some $S_i$ is covered at some point
by the future of a compatible set, then the chosen compatible set $C'$
was the smallest element for $\pc$ verifying this property);
\item \label{condi:deux} if $h(\cro{a}(\cho')) \neq \vide$ (i.e. $\cro{a}(\cho') \in \Comp$), then
$\cho = \cro{a}(\cho')$ (if the whole set $S_i$ is compatible, then we must choose it).
\end{enumerate}
Furthermore, if $I \in \Comp$ we only keep the initial state
of the form $(I, \Hist)$.




\begin{claim} If $S, u,S'$ is a simulation
and $\Co \subseteq Q$ is a compatible set,
then $\cro{u}^{-1}(\Co)$ is a compatible set.
Furthermore if $\cro{u}$ is bijective from $S$
to $S'$, then $|\Comp(S)| \ge |\Comp(S')|$.
\end{claim}

\begin{iproof} The first assertion is obvious
by definition of compatibility and simulations. 
Assume now that $\cro{u}$ is bijective from $S$
to $S'$, then $\cro{u}^{-1}$ induces an injection
from  $\Comp(S')$ to  $\Comp(S)$ by the previous
assertion. Hence $|\Comp(S')| \le |\Comp(S)|$. 
\end{iproof}

Hence we can find
$S_{i+j-1},u_{j} \dots, S_{i+j}$ such that
$|\Comp(S_{i+j-1})| = |\Comp(S_{i+j})|$. It follows 
that $\cro{u}^{-1}$ and $\cro{u}$ are bijections
between $\Comp(S_{i+j-1})$ and $\Comp(S_{i+j})$.




and thus we can extract a simulation
$S_{i-1},u_{i} \dots, S_{i+2^{Q}+1}$ such that
$|S_{i-1}| = \cdots = | S_{i+2^{Q}+1}|$.
Hence the $\cro{u_{i+j}}$ for $1 \le i \le 2^{Q}+1$ are bijections
between these sets.





\subsection{Representing close simulations}

Let $S, u, S'$ be a sub-simulation and
$C' \subseteq S_i$ be a maximal compatible subset.
The function $\pr{u} : S' \rightarrow S$ induces
a function $\pr{u} : C' \rightarrow C \defined \pr{u}(C')$
and   $C,\cro{u},C'$ is a simulation.
We suppose that $C'$ is not \emph{$M |Q|^{|Q|} $}-separable.


Hence by Lemma~\ref{lem:proches} there exists a 
mapping $\beg : C \rightarrow B^*$ (independent
from $u$).

Then for all $q \in Q$ we have $\vava{u}(q) = \alpha_q \beta_q$ where:
\begin{itemize}
\item if $\vava{u}(q) \pref \beg(\pr{u}(q))$, then 
$\alpha_q \defined \vava{u}(q)$ and $\beta_q \defined \movi$;
\item otherwise $\beg(\pr{u}(q)) \pref \vava{u}(q)
\pref \beg(\pr{u}(q)) \alpha$, then $\alpha_q \defined \beg(\pr{u}(q)) $
and $\beta_q$ is such that $\alpha_q \beta_q  = \vava{u}(q)$.
\end{itemize}

Let $\lon{u} \defined \bigwedge_{q \in Q} \beta_q$.
For all $q \in Q$, let $\gamma_q $ be such that
$\beta_q = \lon{u} \gamma_q$.


\begin{claim}
Since $C'$ is not $M |Q|^{|Q|} $-separable, then
$|\gamma_q| \le 2 M |Q|^{|Q|}$.
\end{claim}

\begin{proof}
\gd{TODO}
\end{proof}


Hence we store:
\begin{itemize}
\item the function $\pr{u} : C \rightarrow C'$ in the
state;
\item for $q \in Q$, the values $\alpha_q$ and $\gamma_q$
in the state;
\item $2^{|C|}\times 2^{|C|-1} \times \cdots$ registers containing $\lon{u}$.
\end{itemize}


\subparagraph*{Creating a new close simulation.}

For each $C,a,C'$ where $C'$ is close,
we apply Lemma~\ref{lem:e-beg}, and we build:
\begin{itemize}
\item  a function $\beg : C \rightarrow B^*$ which is 
a beginning for $C$ (stored in the state);
\item for all $q \in C'$, we have that 
$|\pr{a}(q)| \le M$, thus we can compute
$\alpha_q, \lon{a}, \gamma_q$ statically;
\end{itemize}

\subparagraph*{Trimming the simulation.}

If we remove states.
We consider the new maximal compatible
sets of states included in $C$. There are
at most $2^{|C|}$ of them
and they have size at most $2^{|C|-1}$.
Hence we can give $2^{|C|-1} \times \cdots$
registers $\lon{u}$ to each
of them.


Two cases occur:
\begin{itemize}
\item either $\lon{u} = \movi$. In this case,
the informations $\pr{u}(q)$ for $q \in C$ are
completely available in the states.
Thus we can recompute from Lemma~\ref{lem:e-beg},
the $\beg$ and we define $\alpha_q, \lon{a}, \gamma_q$
accordingly;
\item if $\lon{u} \neq \movi$. Then $\beg|_{C'}$
is a beginning for $B \subseteq C$. Furthermore, since
$\beg(\pr{u}(q)) \pref \vava{u}(q)$
for all $q \in C$, it follows that



\begin{claim}
For all simulation $B',v',B''$ a simulation, then there exists
$\alpha' \in B^*$ such that for all $q \in B''$,
$\beg(\pr{v}{q}) \pref \vava{u}(\pr{v}(q))\vava{v}(q) \pref \beg(\pr{v}(q)) \alpha$.
\end{claim}

\begin{proof}
\gd{On utilise le fait qu'on a une égalité compensée.}
\end{proof}

\end{itemize}


\subparagraph*{Merging simulations.}

Let $S,u,S',u',S''$ be a simulation where
$S,u',S''$ is stable. Let $C''$ be a maximal 
compatible subset of $S''$ which is not $M |Q|^{|Q|}$-separable.
Then by stability, $C' \defined \pr{u'}(C'')$ is a maximal
compatible subset of $S'$. It is not $M |Q|^{|Q|}$-separable
by Lemma \gd{todo}.

It follows that $\vava{uu'}(q) = \vava{u}(\pr{u'}(q)) \vava{u'}(q)
= ( \alpha_{\pr{u'}(q)} \lon{u'} \gamma_{\pr{u'}(q)}) (\alpha_{q} \lon{u'} \gamma_{q})$






\begin{lemma}[Compatible states have compatible futures]
Let $p_1, \dots, p_k \in I$ be such that 
$q_1, \dots, q_k \in Q$ be compatible,
there exists $\theta_1, \theta'_1, \dots, \theta_k, \theta'_k \in B^+$ 
such that for all $u \in A^*$, $\alpha_1, \dots, \alpha_k \in B^*$
with $p_i \xrightarrow{u| \alpha_i} q_i$, then
$\alpha_1 \theta_1 {\theta'_1}^\omega
= \cdots = \alpha_k \theta_k {\theta'_k}^\omega $.
In particular $|\alpha_i| \le |\alpha_j| \Rightarrow \alpha_i \pref \alpha_j$.
\end{lemma}


\begin{lemma}[Compatible states have compatible futures]
Let $p_1, \dots, p_k \in I$,
$q_1, \dots, q_k \in Q$ be compatible,
there exists $\theta_1, \theta'_1, \dots, \theta_k, \theta'_k \in B^+$ 
such that for all $u \in A^*$, $\alpha_1, \dots, \alpha_k \in B^*$
with $p_i \xrightarrow{u| \alpha_i} q_i$, then
$\alpha_1 \theta_1 {\theta'_1}^\omega
= \cdots = \alpha_k \theta_k {\theta'_k}^\omega $.
In particular $|\alpha_i| \le |\alpha_j| \Rightarrow \alpha_i \pref \alpha_j$.
\end{lemma}

\begin{proof} By Lemma~\ref{lem:compat}, one has
$v,v'\in A^+$, $q'_1, \dots, q'_k \in Q$, $\beta_1, \beta'_1,\dots, \beta_k,\beta'_k \in B^*$
such that $q_i \xrightarrow{v | \beta_i} q'_i \xrightarrow{v' | \beta'_i} q'_i$
for all $1 \le i \le k$. Assume up to permutation that $q'_1$ is final
then $\theta \defined \beta'_1 \neq \movi$. Let us
now define the words $\theta_i, \theta'_i \in B^*$
for $1 \le i \le k$:
\begin{itemize}
\item if $\beta'_i \neq \movi$, we set $\theta_i \defined \theta_i$ and $\theta'_i \defined \beta'_1$;
\item if $\beta'_i = \movi$, there exists $q''_i \in Q$, $w_i, w'_i \in A^*$
$\gamma_i , \gamma'_i \in B^*$ such that 
$q'_i \xrightarrow{w | \gamma'_i} q''_i \xrightarrow{w | \gamma''_i} q''_i$ 
and $\gamma'_i \neq \movi$. We define $\theta_i \defined \beta_i \gamma_i$
and $\theta'_i \defined \gamma'_i$. 
\end{itemize}
Now if we have $u, \alpha_1, \dots, \alpha_k$ as supposed,
then by Lemma~\ref{lem:continuity-loops}:
$\alpha_1 \theta_1 {\theta'_1}^\omega = \cdots = \alpha_k \theta_k {\theta'_k}^\omega$.
\end{proof}



\begin{lemma} \label{lem:e-beg} Given $S \subseteq Q$, one can
compute a beginning $\beg$ such that
for all simulation $S, u, S'$ with $S'$ compatible, $\exists \alpha \in B^*$
such that $\vava{u}(q) \pref \beg(\pr{u}(q)) \alpha$ for all $q \in Q$.
\end{lemma}

\begin{proof} One can assume that there exists a
simulation $S,u,S'$ with $S'$ compatible (otherwise
the lemma is vacuously true). Hence $S$ is both accessible
and compatible. One can find a simulation
$J, v, S$ with $v \in A^*$, $|v| \le |Q|^{|Q|} $
and $J \subseteq I$. Thus $|\vava{v}(q)| \le M |Q|^{|Q|}$
for all $q \in Q$. Let $\beta \in B^* \defined \bigwedge_{q \in S} \vava{v}(q)$,
it follows from Lemma~\ref{lem:compat} that
$\vava{v}(q)\pref \beta$ for all $q \in Q$. For $q \in S$, define
$\beg(q) \in B^*$ such that $\vava{v}(q) \beg(q) = \beta$.

Now let $S, u, S'$ be any simulation such
that $S'$ is compatible. Then we have a run of the form
$\pr{v}(\pr{u}(q)) \xrightarrow{v | \vava{v}(\pr{u}(q))} \pr{u}(q) \xrightarrow{u | \vava{u}(q)} q$
for all $q \in S'$.
Let $\gamma \in B^*$ be the longest of the $\vava{v}(\pr{u}(q)) \vava{u}(q)$,
since $S'$ is compatible it follows from
Lemma~\ref{lem:compat} that $\vava{v}(\pr{u}(q)) \vava{u}(q) \pref \gamma$
for all $q \in S'$. Thus in particular $\beta \pref \gamma$
since $\pr{u}$ is surjective, so let $\alpha \in B^*$ be such that $\beta \alpha = \gamma$.
Hence $ \vava{v}(\pr{u}(q)) \vava{u}(q) \pref \gamma = \beta\alpha =
\vava{v}(\pr{u}(q)) \beg(\pr{u}(q))  \alpha$
and finally $\vava{u}(q) \pref \beg(\pr{u}(q))  \alpha$.
\end{proof}





\begin{lemma}
Let $S,u,S'$ be a simulation such that $S'$ is compatible.
Then there exists a function $f : S' \rightarrow B^*$
such that $\pre{u}{S,S'}(q)f(q) = \pre{u}{S,S'}(p)f(p)$
for all $p,q \in Q$.
\end{lemma}

\begin{lemma}
Let $S,u,S'$ be a $M|Q|^{|Q|}$-separable
simulation such that $S'$ is compatible.
Then there exists a function $f : S' \rightarrow B^*$
such that $\pre{u}{S,S'}(q)f(q) = \pre{u}{S,S'}(p)f(p)$
for all $p,q \in Q$.
\end{lemma}







\begin{definition}  \label{def:beg}
Let $S \subseteq Q$, we say that a 
function $\beg: S \rightarrow B^*$
is a \emph{beginning for $S$} if
$|\beg(q)| \le M |Q|^{|Q|}$ for all $q \in S$,
and if there exists a simulation $J,u,S$
with $J \subseteq I$ such
that for all $p,q \in S$, $\vava{u}(p) \beg(p) = \vava{u}(q) \beg(q)$.
\end{definition}






A first idea is to
store directly the value $\trans^x_i(\reg)$ in a register
when in position $i \ge 1$ of $x \in A^\omega$.
Indeed, due to the $1$-bounded behavior, $\trans^x_i(\reg)$
can only be used once in $\out$ (at some point in the future).
However, it is not possible to maintain this information in a copyless fashion,
since if $\trans$ e.g. performs the substitution
$\reg \mapsto \reg, \regg \mapsto \reg$,
we are unable to determine if the value of $\reg$
should be used to compute that of $\reg$ of that of $\regg$.


\subparagraph*{Storing substitutions along portions of runs.}
In order to build our copyless \SST{}, we shall keep in memory
some  \emph{copyless substitutions applied along portions of the run of $\trans$}.
If the substitution applied when reading $x[i{+}1]$ makes copies, we memorize it separately.
We show how to maintain this abstraction using only a finite
number of states and registers.

\begin{definition} Given $s \in \subst{\Regs}{B}$, we define its
\emph{used set} as the set of ``old registers'' which are used
by $s$, that is $\Used{s} \defined \{\reg \in \Regs : \reg \text{ occurs in } s(\regg) \text{ for some } \regg \in \Regs \}$.
\end{definition}


We introduce the notion of \emph{decomposition} of the substitution $\trans^x_i$,
which is a way to split it into several substitutions
which only keep the ``useful'' information. This is the
abstraction we want to keep track of when in position $i \ge 0$
if input $x \in A^\omega$.


Note that if $s_{\ell} \in \subst{\vide}{B}$, then its extension
to words in $(\vide \uplus B)^*$ is just the identity function
over $B^*$. We can easily recover $\trans^x_i$ from its decomposition,
as shown below.

\begin{claim} If $s_1,\dots, s_n$ is a decomposition
of $\trans^x_i$, then $s_1 \circ \dots \circ s_n = \trans^x_i$.
\end{claim}

\begin{proof} We have  $s_1 \circ \dots \circ s_n(\reg)
= \lambda(\delta(q_0, x[1{:}i_1])) \circ \cdots \circ \lambda(\delta(q_0, x[1{:}i_{m-1}], x[i_{m-1}{+}1{:}i])(\reg)$
which corresponds to the definition of $\trans^x_i(\reg)$.
\end{proof}

\begin{claim}[Long decompositions have copyless substitutions]
Let $x \in A^\omega$ and $i \ge 1$ such that
$\trans^x_i$ is defined. If $s_1, \dots, s_m$
is a decomposition of $\trans^x_i$ with $m \ge \gd{}$,
then there exists $1 \le \ell \le m-1$ such that $s_{\ell}$ and $s_{\ell+1}$ are copyless.
\end{claim}

\fin

\begin{proof} 
Let $i_0, \dots, i_m$ be given by Definition~\ref{def:decompose}.
It follows from this definition that for $1 \le \ell'  \le \ell \le m$,
$s_{\ell, \ell'} \defined s_\ell \circ \cdots \circ s_{\ell'}$
is the restriction of $ \lambda(\delta(q_0, x[1{:}i_{\ell'}]), x[i_{\ell'}{+}1{:}i_{\ell}])$
to $\Dom{s_{\ell}}$.
Given $1 \le \ell \le m$, we say that $R \subseteq \Dom{s_{\ell}}$
is \emph{free} in 
\emph{share information in $\ell$} if there exists
$1\le \ell' \le \ell$ such that there exists $\regg \in \Regs$
such that $\regg$ occurs both in $s_{\ell', \ell}(\reg_1)$
and $s_{\ell', \ell}(\reg_2)$.
Let us define by $K_{\ell}$ the number of tuples
$(\reg_1, \reg_2)$ which share

We claim that the following properties hold for $1 \le \ell \le m{-}1$:
\begin{itemize}
\item $K_{\ell} \le K_{\ell+1}$. Indeed, consider a function
$f : \Dom{s_{\ell}} = \Used{s_{\ell+1}} \rightarrow \Dom{s_{\ell+1}}$
such that $\reg$ occurs $s_{\ell+1}(f(\reg))$
(such a function exists due to the definition of $\Used{s_{\ell+1}}$).
It is clear that if $\reg_1, \reg_2 \in \Dom{s_{\ell}}$ share information in $\ell$,
then $f(\reg_1), f(\reg_2)$ share information in $\ell{+}1$.
Furthermore, if $\reg'_1, \reg'_2 \in \Dom{s_{\ell}}$ also share information in $\ell$,
we have $(f(\reg_1), f(\reg_2)) \neq (f(\regg))$
\item if $s_{\ell+1}$ is not copyless, then $K_{\ell} < K_{\ell + 1}$.
\end{itemize}
 
Since $\trans$ is $1$-bounded, there are at most
$K$ occurences of each $\reg \in \Regs$ in $\{s_{\ell, \ell'}(\regg) : \regg \in \Regs\}$.


$q_0, \dots, q_i $We now that $\lambda()()$ the converse, that is 

\end{proof}



\subparagraph*{Update when reading a letter.}
Assume that we read a new substitution $s$.
We do the following operations:
\begin{itemize}
\item use the new set of substitutions
\end{itemize}







\section{Simulation}

Assume we are given as input when $x \in \Dom{f}$ a sequence
of compatible sets $C_0, C_1, \dots$ verifying
the properties of Proposition~\ref{prop:pre-compat}.

If $C_i$ is the current compatible, we keep
track of the following information:
\begin{itemize}
\item for all subset of two elements
 $\{q,q'\} \subseteq C_i$
remember: either that they are $K$-remote,
or if they are $K$-Far;
\item \gd{something} for all $q$ compatible.
\end{itemize}

The idea is that we simulate all the possible runs
reading $u_1 \cdots u_n$ from $S_0$ (hence the
condition on the images) without keeping track of the deadlocks
(hence totality).

We say that the step $S,t,T$ is \emph{bijective} if $\pre{t}{S,T}$ is so.

\begin{lemma} Let $S_0, u_1, S_1, \dots, u_n, S_n$ be
a simulation with $n > |Q|$. Then there exists $1 \le i \le n$ such that
$S_{i-1}, u_i, S_i$ is stable.
\end{lemma}

\begin{proof} Since $\trans$ is trim and unambiguous,
for all $1 \le i \le n$ and for all $q,q' \in S_{i-1}$
we have $(\push{u_i}{\{q\}}) \cap (\push{u_i}{\{q'\}}) = \vide $.
Since $u_i$ is total, we thus get $|Q| \ge |\push{u_i}{S_{i-1}}| \ge |S_{i-1}|$.
Hence there exists $1 \le i \le n$ such that
$|S_{i-1}| = |S_i|$ which implies that 
$u_i$ is a bijection between these sets
(by definition of steps and unambiguity).
\end{proof}



\subsection{Representation of a simulation}

Let $x \in \Dom{f}$ and $m \ge 0$ and assume that we have read
the input up to letter $m$, that is we have read
$C_0 (x[1], C_1) \cdots (x[m],C_m)$.
Then we keep track of the following elements:
\begin{itemize}
\item a simulation $S_0, u_1, S_1, \dots, S_n$
such that $n \le |Q|$, $S_n = C_m$
and $u_1 \cdots u_n = x[1{:}m]$ and $S_n = C_m$;
\item the global information:
\begin{itemize}
\item a register $\out$ which contains some information;
\item a word $\alpha_q \in B^*$ for all $q \in S_n$
\gd{bounded and stored in the state};
\end{itemize}
\item the step information,
for all $1 \le i \le n$, for all $\chain \in \Chains(S_i)$:
\begin{itemize}
\item  for all $q \in \Supp(\chain)$,
a bit $b_q \in \{0,1\}$ (charged or not);
\item a register $\reg_\chain$ (the common).
\end{itemize}
\end{itemize}

\begin{definition} Let $C \in \Comp$. Given $\ell \ge 1$,
we say that $\chain = (q_1, \dots, q_{\ell}) \in C^{\ell}$ is a $C$-\emph{chain}
if the $q_i$ are distinct and the \emph{support}
$\Supp(\chain) \defined  C \smallsetminus \{q_1, \dots, q_{\ell}\}$
is not empty.
\end{definition}

We denote by $\Chains(C)$ the set of all $C$-chains.

\begin{example} If $C = \{1,2,3\}$, the $C$-chains
are $(1), (2), (3), (1,2), (1,3), (2,1), (2,3)$, $(3,1), (3,2)$
and we have $\Supp(1) = \{2,3\}$ and $\Supp(1,2) = \{3\}$.
\end{example}





\begin{lemma} 
During the simulation, the following holds.
For all $q_n \in S_n$, if the unique run from $I$ to $q_n$ is
(with $q_i \in S_i$):
$ q_0 \runs{u_1 | \alpha_1} q_1 \runs{} \cdots \runs{} q_n$
\begin{itemize}
\item either there is a first time $S_k$
when there is a separation. Then 
for all $k \le i \le n$, if $\chain_i$ is an $S_i$-chain,
then:
$$\alpha_1 \cdots \alpha_n = \out b_{\chain_k} \reg_{\chain_k} \cdots b_{\chain_n} \reg_{\chain_n} \alpha_{q_n}$$
\item or there is no separation. In
that case we have
$$\alpha_1 \cdots \alpha_n = \out  \alpha_{q_n}$$
\end{itemize}
\end{lemma}



\subsection{Operations on simulations}

Let $S_0, u_1, S_1, \dots, S_n$ be the current simulation.
We have by induction hypothesis that $S_n = C_i$.
We assume that $C_{i+1}$ is given by the machine.
Then $C_{i+1} \subseteq \push{x[i{+}1]}{S_n}$.
In order to force an equality, we first trim.
Then, we add the letters.


\subparagraph*{Trim.} We remove some states of $S_n$
while preserving the invariants.

\subparagraph*{Adding a new letter.} 
Now we exactly have $C_{i+1} = \push{x[i{+}1]}{S_n}$
and we can add a letter. We define $S_{n+1} \defined C_{i+1}$.
Two cases occur :
\begin{itemize}
\item either $S_{n}$ is ``far''. In that case, we have
some $\theta$ (which corresponds to the $\theta$
from before it was already ``far'' by \gd{some Lemma}).

For all $q \in S_{n+1}$ we have a unique $q' \in S_n$
such that $q' \runs{a | \alpha} q$. We define
$\alpha_q \leftarrow \alpha_{q'}\alpha$. 
But if $\theta^{\ell} \pref \alpha_q$, we define $\alpha_q \leftarrow {\theta^{-\ell}} \alpha_q$
and $b_q \leftarrow b_q + \ell$. Then we do the ``descent''.

It is easy to see that the invariants are preserved.


\item or $S_{n}$ is ``close''. In this case,
we had that $\out$ contained
the longest common prefix and the $\alpha_q$
contain the \gd{petit bouts}. There is no problem,
we can still contain this prefix.
\end{itemize}


\subparagraph*{Merging.}





\begin{vieux}
let $r \in T$ be such that $|\val{t}{S,T}(r)|$ is maximal,
we define the \emph{delay} function $\del{t}{S,T} : T \rightarrow B^*$
by $\del{t}{S,T}(q)  = (\val{t}{S,T}(q))^{-1}  \val{t}{S,T}(r)$ for $q \in T$.
\end{vieux}



\begin{vieux}
\begin{lemma}[Ends 3] \label{lem:ends3}
Let $J,u,C, v, D$ be an initial sequence of steps,
and $r \in D$ be such that $|\val{J,C}{u}(\pre{C,D}{v}(r))|$
is maximal, then for all $q \in D$:
$$
\val{C,D}{v}(q) \en{D}(q)
= \del{t}{S,T}(\pre{u}{T,U}(q)) \val{u}{T,U}(r) \en{U}(r).
$$
\end{lemma}


\begin{proof} Immediate from Lemma~\ref{lem:ends2}
by choosing $p =r$ and using the definition of $\del{}{}$.
\end{proof}

\end{vieux}




























\begin{vieux}

\begin{lemma} \label{lem:theta} Let  $T \in \Comp$  be separable
and $S,t,T$ be an initial step. There exists 
$\theta \in B^*$ depending only on $T$ and $\del{t}{S,T}$,
such that $|\theta| = \Bound!$ and for all step $T,u,U$ and $q \in U$:
\begin{equation*}
\val{u}{T,U}(q) \en{U}(q) = \del{t}{S,T}(\pre{u}{T,U}(q)) \theta^\omega
\end{equation*}
\end{lemma}

\begin{proof} Since $T$ is separable, we get $\pu,\qu \in T$ verifying the conditions
of Lemma~\ref{lem:carac-separ}. Assume by symmetry that
$|\beta'(\pu)| > |\beta'(\qu)|$. We have $0 <|\beta'(\pu)| \le M \bound = \Bound$,
hence by pumping the loop we can assume that $|\beta'(\pu)| = \Bound!$.
Let $J \defined i(T)$, then
for all $n \ge 0$, $J, v{v'}^nv'', T$ is an initial step.
Furthermore for $n \defined |\beta'(\pu)|k$ and $k \ge 0$ large enough, we get:
\begin{equation}
\label{eq:abo}
\begin{aligned}
\left(\val{v{v'}^nv''}{J,T}(q)\right)^{-1} \val{v{v'}^nv''}{J,T}(\pu)
&= \left(\beta(\qu) \beta'(\qu)^n \beta''(\qu)\right)^{-1} \beta(\pu) \beta'(\pu)^n \beta''(\pu)\\
&=  \left(\beta(\pu) \beta'(\qu)^n \beta''(\pu)\right)[|\beta(\qu)\beta''(\pu)| + k |\beta'(\pu)\beta'(\qu)| : ]\\
&= \left(\beta'(\pu)^{k(|\beta'(\pu)| {-} |\beta'(\qu)|)}\beta''(\pu)\right) [K :] \\
& \substack{~~\tnorm{with}~~ K \defined |\beta(q)\beta''(\qu)| {-} |\beta(\pu)|}\\
&= \gamma^{k-K} \delta(k)
\end{aligned}
\end{equation}
if we define $\gamma$ as a conjugate of $\beta'(\pu)$:
\begin{equation*}
\gamma \defined (\beta'(\pu)^\omega) [K: K {+} |\beta'(\pu)|]
\end{equation*}
which only only depends on $T$,
and $\delta(k) \defined \left(\gamma^{k-K})^{-1} \left(\beta'(\pu)^{k(|\beta'(\pu)| - |\beta'\qu|)} \beta''(\pu)\right)
[K{:}] \right)$.

Now let $\widetilde{\pu}$, $\widetilde{\qu}$ be such that
$\pre{u}{T,U}(\widetilde{\pu}) = \pu$ and $\pre{u}{T,U}(\widetilde{\qu}) = \qu$.
We get from Lemma~\ref{lem:ends2}:
\begin{equation*}
\begin{aligned}
\val{u}{T,U}(\widetilde{\qu}) \en{U}(\widetilde{\qu})
&= \left(\val{v{v'}^nv''}{J,T}(\qu)\right)^{-1} \val{v{v'}^nv''}{J,T}(\pu) \val{u}{T,U}(\widetilde{\pu}) \en{U}\\
& = \gamma^{k-K} \delta(k) \val{u}{T,U}(\widetilde{\pu}) \en{U}(\widetilde{\pu})
\substack{\tnorm{~~by Equation~\ref{eq:abo} for $k \ge 0$ large enough }}
\end{aligned}
\end{equation*}
By using arbitrarily large $k$, we see that
$\val{u}{T,U}(\widetilde{\qu}) \en{U}(\widetilde{\qu}) = \gamma^{\omega}$
(which only depends on $T$).

Now we consider the simulation $S,t,T,u,U$. Let $r \in U$ be such that 
$|\val{t}{S,T}(\pre{u}{T,U}(r))|$ is maximal, by Lemma~\ref{lem:ends3}
we have:
$$
\gamma^\omega = \val{u}{T,U}(\widetilde{\qu}) \en{U}(\widetilde{\qu})
= \del{t}{S,T}(\qu) \val{u}{T,U}(r) \en{U}(r).
$$
and so $\del{t}{S,T}(\qu) \val{u}{T,U}(r) \en{U}(r) =
(\gamma^\omega)[|\del{t}{S,T}(\qu)|:] = \theta^\omega$
by defining:
\begin{equation*}
\theta \defined (\gamma^\omega)[|\del{t}{S,T}(\qu)|:|\del{t}{S,T}(\qu)|+|\gamma|]
\end{equation*}
which only depends on $\gamma$ (i.e. $T$), $\qu$ (i.e. $T$) and $\del{t}{S,T}$.

Finally we apply Lemma~\ref{lem:ends3} once more and get for all $q \in U$:
$$
\val{u}{T,U}(q) \en{U}(q)
= \del{t}{S,T}(q) \val{u}{T,U}(r) \en{U}(r) =  \del{t}{S,T}(q) \theta^\omega.
$$
\end{proof}





In particular we get \framebox{$\val{T,U}{u}(q) \pref  \del{t}{S,T}(\pre{u}{T,U}(q)) \theta^\omega$}.


\end{vieux}




\begin{vieux}
\begin{proof}
By Lemma~\ref{lem:ends}, all the $\val{t}{S,T}(q) $
must be prefixes of each other.
\end{proof}
\end{vieux}








\begin{definition}[Extension] Let $f,g: A^\omega \parfonc B^\omega$
 be two partial functions. We say that $g$ \emph{extends} $f$
 whenever $\Dom{f} \subseteq \Dom{g}$ and $\forall x \in \Dom{f}$,
 $f(x) = g(x)$.
\end{definition}
















\begin{claim} After this operation, we  have:
\begin{itemize}
\item $\val{x[1{:}i]}{J',C'}(q) = \out \alpha_q$ for all $q \in C'$;
\item the $\alpha(q)$ for $q \in C'$ are mutual prefixes, so $\alpha = \bigvee_{q \in C'} \alpha_q$ is defined;
\item for all $q \in C' $, $\del{x[1{:}i]}{J',C'}(q)$ from  Definition~\ref{def:del} is $\alpha(q)^{-1} \alpha$.
\end{itemize}
\end{claim}
%
The end of the construction depends on wether $C'$ is separable or not:
\begin{itemize}
\item if $C'$ is not separable, then we must have $|\alpha_q| \le \Bound$.
We set $\lag(q) \becomes \alpha(q)$ for all $q \in C'$
and our \DSST{} goes into its non-separable mode.
The invariants of this mode hold;
\item if $C'$ is separable, then by Lemma~\ref{lem:theta} we have
for all step $C', u, D'$ and for all $q \in D'$ that
$\val{u}{C',D'}(q) \en{D'}(q) = \del{x[1{:}i]}{J',C'}(\pre{u}{C',D'}(q)) {\theta'}^\omega
= \alpha(\pre{u}{C',D'}(q))^{-1} \alpha {\theta'}^\omega$.

But since we have 
\gd{utiliser une autre del pour un autre truc plus court,
et comparer.}
\gd{Faire un lemme extérieur dans la partie d'avant qui permet de créer du $\theta$
lorsqu'on est loin.}

\end{itemize}






\fin

And so: $ \out~\lagm ~
\theta^{n} \last(q) = \val{x[1{:}i]}{\Jf',\Cf'}(q)
\pref \com{J',E}{x[1{:}j]} \tau \phi^\omega$.


 exists $q \in C'$ which is not lagging by invariant~\ref{inv:lagging}
and because $\pi = \Cf C'$ is close. Let us consider the longest such $q'$,
Furthermore, we have $\val{J',C'}{x[1{:}i]}(q') = \out \lagm  \theta^{n} \last(q')$
for some $n > 0$. But since it is the longest,
we can show that $\com{J',E}{x[1{:}j]} \advm{J',E}{x[1{:}j]} \pref
\out \lagm  \theta^{n} \last(q') \pref \com{J',E}{x[1{:}j]} \lag \phi^\omega$
and so we show that \gd{renversement.}


But $\val{E,D}{x[j{+}1{:}i]u}(q) = \val{E,\Cf'}{x[j{+}1{:}i]}(\pre{\Cf',D}{u}(q))\val{\Cf',D}{u}(q)$
so finally:
$$
\val{\Cf',D}{u}(q) \pref (\val{E,\Cf'}{x[j{+}1{:}i]}(\pre{\Cf',D}{u}(q)))^{-1}
(\adv{\Jf,E}{x[1{:}j]}(\pre{E,D}{x[j{+}1{:}i]u}(q)))^{-1} \tau  \phi^\omega
$$
but this should be 

\begin{vieux}
Let $c \defined \bigwedge_{q \in C'} \lag(q)$,
we update $\out \becomes \out c \outi{\Cf C'}$
and for all $q \in C'$, $\lag(q) \becomes c^{-1} \lag(q)$
and $\last(q) \becomes \theta^{\nb{\Cf}(q)} \last(q)$.
Then, we update $\nb{C' \pi} \becomes \nb{\Cf C' \pi}$
and $\outi{C' \pi} \becomes \outi{\Cf C' \pi}$
for all $\pi \in (C')^{-1}\tree{C'}$ 
(except $\pi = \movi$, in which case we do not modify $\outi{C'}$).
We finally update $\Jf \becomes \pre{\Jf, \Cf}{x[1{:}i]}(C')$
and $\Cf \becomes C'$.
\end{vieux}

and so in particular we have $\adv{J',C'}{x[1{:}j]}(q_1) \pref  \advm{J',E}{x[1{:}j]} \pref \lag  \phi^\omega$
but since $|\advm{J',E}{x[1{:}j]}| \ge |\adv{J',E}{x[1{:}j]}(q_1)| > \gd{} \Bound!$, then we deduce
that $\advm{J',E}{x[1{:}j]} = \lag \gamma$ with $\gamma > \gd{}$ and $\gamma \pref \phi^\omega$.

































\subsection{Essai 1}


Denote by $\cro{\nb{\pi}}_{i}, \cro{\outi{\pi}}_i$ the 
configuration of $\strans$ after reading $C^x_i$.

\begin{sublemma} \label{slem:infini} Let $N \le i_1 \le i_2$. Let $S_1 \subseteq C^x_{i_1}$, be such that
$S_1, x[i_1{+}1{:}i_2], C^x_{i_2}$ is a step.
Let $q_2 \in S_2$ be such that $\cro{\nb{C^x_{i_2}}(q_2)}_{i_2} = 0$
and $q_1 \defined \pre{C^x_{i_1},C^x_{i_2}}{x[i_1{+}1{:}i_2]}(q_2)$.
Then:
\begin{enumerate}
\item \label{it:i1} there exists $D_1 \cdots D_{n} \in \tree{C^x_{i_1}}$
such that $D_n = S_1$ and:
\begin{itemize}
\item $\cro{\nb{D_1 \cdots D_j}}_{i_1}(q_1) = 0$ for all $1 \le j \le n$;
\item $ \cro{\outi{D_1 \cdots D_j}}_{i_1} = \movi$ for all $2 \le j \le n$;
\end{itemize}
\item \label{it:i2}
$|\val{C^x_{i_1},C^x_{i_2}}{x[i_1{+}1{:}i_2]}(q_2)| = |\cro{\last}_{i_2}(q_2)| - |\cro{\last}_{i_1}(q_1)|
+ |\cro{\lag}_{i_2}(q_2)| - |\cro{\lag}_{i_1}(q_1)|$.
\end{enumerate}
\end{sublemma}


\paragraph{Proof of Lemma~\ref{lem:lazy}}

The result is shown by a decreasing induction on
$i_1 \le i_2$. The base case is trivial, let us show
it for $i_0 \defined i_1{-}1$. Let $S_0 \subseteq C^x_{i_0}$
be such that $S_0, x[i_0{+}1{:}i_2], C^x_{i_2}$ is a step.
Let $S_1 \defined \pre{C^x_{i_1}, C^x_{i_2}}{x[i_1{+}1{:}i_2]} (C^x_{i_2})$,
then $S_0, x[i_1], S_1$ and $S_1, x[i{+}1{:}i_2], C^x_{i_2}$ are two steps.

Let $q_2 \in C^x_{i_2}$ be such that $\cro{\nb{C^x_{i_2}}(q_2)}_{i_2} = 0$
and $q_1 \defined \pre{C^x_{i_1},C^x_{i_2}}{x[i_1{+}1{:}i_2]}(q_2)$.
By induction hypothesis, we have \ref{it:i1} (for some $D_1 \cdots D_n$)
and~\ref{it:i2} from Sublemma~\ref{slem:infini}.
Now let us consider the transition of $\strans$
from $C^x_{i_0}$ to $C^x_{i_1}$. It obtained by possibly
applying Subsubsection~\ref{sssec:prepro}
(in the ``non-close'' case)
and then Subsubsection~\ref{sssec:up-step}.
We study the preservation of our property along
these operations,
from the last to the first one.

\subparagraph*{Last operation: applying Subsection~\ref{ssec:tool} in Subsubsection~\ref{sssec:up-step}.}
Let $\nb{\pi}', \outi{\pi}'$, etc.
denote the configuration of $\strans$ right after Lemma~\ref{lem:sim:prune}
in Subsubsection~\ref{sssec:up-step}.
Since Algorithm~\ref{algo:down}
cannot empty some register,
we necessarily had $\outi{D_1 \cdots D_j}' = \movi$ for all $2 \le j \le n$.
Since for all $1 \le j \le n$, we have
$\cro{\nb{D_1 \cdots D_j}}_{i_1} = 0$ and
$\outi{D_1 \cdots D_j}' = \cro{\outi{D_1 \cdots D_j}}_{i_1}$ is not modified,
we had $\nb{D_1 \cdots D_j}'(q_1) = 0$.
In particular, $\nb{C^x_{i_1}}(q_1)$ is not modified,
hence we had $n(q_1) = 0$ and so $\last'(q_1) = \cro{\last(q_1)}_{i_1}$.
Furthermore, $\lag'(q_1) = \cro{\lag(q_1)}_{i_1}$.


\subparagraph*{Previous operation: beginning of Subsubsection~\ref{sssec:up-step}.}
Now let $\nb{\pi}'', \outi{\pi}''$, etc.
 denote the configuration of $\strans$ before applying the whole
 Subsubsection~\ref{sssec:up-step}.
The operation builds $1 = k_1 < \cdots < k_{m} \le n$
and $C_1 \cdots C_{m}$ such that $C_j = \pre{a}{\Cf, C^x_{i}}(D_{k_j})$.
We first note that $C_{k_{m}} = \pre{\Cf, C^x_{i_1}}{x[i_1]}(S_1) 
= \pre{C^x_{i_0}, C^x_{i_1}}{x[i_1]}(S_1) = S_0$ since $S_0, x[i], S_1$ is a step.\\
Let us consider $C_1 \cdots C_j \in \tree{\Cf}$ for some $1 \le j \le n$. By construction
we have:
\begin{itemize}
\item $\outi{C_1 \cdots C_j}'' = \outi{D_1 \cdots D_{i_j}}' = \movi$ if $2 \le j \le n$;
\item $\nb{D_1 \cdots D_j}' = \nb{C_1 \cdots C_j}'' \circ \pre{\Cf, C^x_{i_1}}{x[i_1]}$.
Thus $ \nb{C_1 \cdots C_j}''(q_0) = 0$ if $q_0 \defined \pre{\Cf, C^x_{i_1}}{x[i_1]}(q_1)$
\end{itemize}
Finally, we note that $c = \movi$ since there is no output.
As a consequence, it is quite easy to see that $|\val{S,\new{S}}{x[i{+}1{:}\new{i}]}(q_1)| = |\last'(q_1)| - |\last''(q_0)|
+|\lag'(q_1)| - |\lag''(q_0)|$.


\subparagraph*{Previous operation: Subsubsection~\ref{sssec:prepro}.}
If Subsubsection~\ref{sssec:prepro} was not used,
the proof is completed. 

\gd{todo @HERE}



Otherwise,
 let $\nb{\pi}''', \outi{\pi}'''$, etc.
 denote the information of $\strans$ right after Lemma~\ref{lem:sim:prune}).
Thanks to the above proof (and by a similar study of Algorithm~\ref{algo:down}),
we see that $\nb{\rho}'''(p) =0$, $\outi{C_1 C_2}''' = \cdots = \outi{C_1 \cdots C_n}'''= \movi$
and:
\begin{equation} 
\label{eq:labelle}
\begin{aligned}
|\val{S,\new{S}}{x[i{+}1{:}\new{i}]}(q)| = &|\new{\last(q)}| - |\last'''(p)|
+ |\new{\lag(q)}| - |\lag''''(p)| \\
&+ \Bound! \times \left( \sum_{j=1}^n \new{\nb{D_1 \cdots D_j}(q)} - \sum_{j=1}^m \nb{C_1 \cdots C_j}'''(p)\right)
\end{aligned}
\end{equation}
Let us finally consider the beginning of Subsubsection~\ref{sssec:prepro}.
Since there is no output, $c = \movi$ and $\lag(q) = \lag'''(q)$.
Let $\phi \defined C^x_i C_1 \cdots C_n \in \tree{C^x_i}$.
We had $\outi{C^x_i C_1} = \movi$ (by construction
and since there is no output) and $\outi{C^x_i C_1 \cdots C_j} = \outi{C_1 \cdots C_j}''' = \movi$
for all $j \ge 2$. Furthermore $\nb{\phi}(p) = \nb{\rho}'''(p) = \movi$.
Finally note that $|\last'''|(q) - |\last(p)| = \Bound! \nb{C^x_i}(q)$
and $\nb{C^x_i C_1 \cdots C_j}(p) = \nb{C_1 \cdots C_j}'''(p)$
for $j \ge 1$. This concludes the proof
by using Equation~\ref{eq:labelle}.





\subsection{Essai 2}


Denote by $\cro{\nb{\pi}}_{i}, \cro{\outi{\pi}}_i$ the 
configuration of $\strans$ after reading $C^x_i$.

\begin{sublemma} \label{lem:lazy} Let $N \le i_1 \le i_2$.
 Let $S_1 \subseteq C^x_{i_1}$,
$S_2 \subseteq C^x_{i_2}$ be such that
$S_1, x[i_1{+}1{:}i_2], S_2$ is a step
and for all $C^x_{i_2} \supseteq T \supsetneq S_2$,
we have $\pre{ C^x_{i_1}, C^x_{i_2}}{x[i_1{+}1{:}i_2]}(T) \neq S $
Let $\pi = D_1 \cdots D_{n} \in \tree{C^x_{i_2}}$
with $S_2 = D_n$ be such that
$\cro{\outi{D_1 D_2}}_{i_2} = \cdots = \cro{\outi{D_1 \cdots D_n}}_{i_2} = \movi$.
Let $q_2 \in S_2$ be such that $\cro{\nb{\pi}(q_2)}_{i_2} = 0$
Let $q_1 \defined \pre{S,\new{S}}{x[i_1{+}1{:}i_2]}(q_2)$,
then there exists $\rho = C_1 \cdots C_{m} \in \tree{C^x_{i_1}}$
with $C_m = S$, such that $\cro{\outi{C_1 C_2}}_{i_1} =
\cdots = \cro{\outi{C_1 \cdots C_m}}_{i_1} = \movi$,
$\cro{\nb{\rho}}_{i_1}(q_2) = 0$, and:
\begin{equation*} 
\begin{aligned}
|\val{C^x_{i_1},C^x_{i_2}}{x[i_1{+}1{:}i_2]}(q_2)| = &|\cro{\last}_{i_2}(q_2)| - |\cro{\last}_{i_1}(q_1)|
+ |\cro{\lag}_{i_2}(q_2)| - |\cro{\lag}_{i_1}(q_1)| \\
&+ \Bound! \times \left( \sum_{j=1}^n \cro{\nb{D_1 \cdots D_j}}_{i_2}(q_2)
- \sum_{j=1}^m \cro{\nb{C_1 \cdots C_j}}_{i_1}(q_1)\right).
\end{aligned}
\end{equation*}
\end{sublemma}


\paragraph{Proof of Lemma~\ref{lem:lazy}}

The result is shown by a decreasing induction on
$i_1 \le i_2$.  Assume that we have
shown the result for some $i_1 \le i_2$, we
show it for $i_0 \defined i_1{-}1$. Let $S_0 \subseteq C^x_{i_1-1}$
and  $S_2 \subseteq C^x_{i_2} $ be such that
$S_0, x[i_1{:}i_2], S_2$ is a step.
Let $S_1 \defined \pre{C^x_{i_1}, C^x_{i_2}}{x[i_1{+}1{:}i_2]} (S_2)$,
then $S_0, x[i_1], S_1$ and $S_1, x[i{+}1{:}i_2], S_2$ are two steps.
Consider some $C^x_{i_2} \supseteq T \supsetneq S_2$,
then $\pre{ C^x_{i_0}, C^x_{i_2}}{x[i_1{+}1{:}i_2]}(T) \neq S_1$
(indeed the converse would imply $\pre{ C^x_{i_0}, C^x_{i_2}}{x[i_1{:}i_2]}(T) = S_0$,
which is a contradiction).

Let $\pi = D_1 \cdots D_{n} \in \tree{C^x_{i_2}}$
with $S_2 = D_n$ be such that
$\cro{\outi{D_1 D_2}}_{i_2} = \cdots = \cro{\outi{D_1 \cdots D_n}}_{i_2} = \movi$.
Let $q_2 \in S_2$ be such that $\cro{\nb{\pi}(q_2)}_{i_2} = 0$.
By induction hypothesis, if $q_1 \defined \pre{S,\new{S}}{x[i_1{+}1{:}i_2]}(q_2)$,
then there exists $\rho = C_1 \cdots C_{m} \in \tree{C^x_{i_1}}$
with $C_m = S$, such that $\cro{\outi{C_1 C_2}}_{i_1} =
\cdots = \cro{\outi{C_1 \cdots C_m}}_{i_1} = \movi$,
$\cro{\nb{\rho}}_{i_1}(q_2) = 0$, and:
\begin{equation*} 
\begin{aligned}
|\val{C^x_{i_1},C^x_{i_2}}{x[i_1{+}1{:}i_2]}(q_2)| = &|\cro{\last}_{i_2}(q_2)| - |\cro{\last}_{i_1}(q_1)|
+ |\cro{\lag}_{i_2}(q_2)| - |\cro{\lag}_{i_1}(q_1)| \\
&+ \Bound! \times \left( \sum_{j=1}^n \cro{\nb{D_1 \cdots D_j}}_{i_2}(q_2)
- \sum_{j=1}^m \cro{\nb{C_1 \cdots C_j}}_{i_1}(q_1)\right).
\end{aligned}
\end{equation*}


Now let us consider the transition of $\strans$
from $C^x_{i-1}$ to $C^x_i$. It obtained by possibly
applying Subsubsection~\ref{sssec:prepro}
(in the ``non-close'' case)
and then Subsubsection~\ref{sssec:up-step}.

\subparagraph*{Last operation: applying Subsection~\ref{ssec:tool}.}
Let $\nb{\pi}', \outi{\pi}'$, etc.
be the information of $\strans$ before applying  Subsubsection~\ref{sssec:up-step}
for the end of Subsubsection~\ref{sssec:up-step}
(this is the last operation which is applied in the transition).
Since Algorithm~\ref{algo:down}
cannot empty a register $\outi{C_1 \cdots C_j}$,
we necessarily had $\outi{C_1 C_2}' = \cdots = \outi{C_1 \cdots C_m}' = \movi$.
Since $\cro{\nb{\rho}(q_1)}_{i_1} = 0$ and $\outi{\pi}' = \cro{\outi{\pi}}_{i_1}$ is unchanged,
we have $\nb{\pi}(q_1)' = 0$,
and $\nb{\pi\{q\}}'(q_1) = \cro{\nb{\pi\{q\}}}_{i_1}(q_1)$.
By using the fact that Subsection~\ref{ssec:tool}
preserves invariant~\ref{inv:past}, we conclude
that:
\begin{equation*} 
\begin{aligned}
0 &= |\cro{\last}_{i_1}(q_1)| - |\last'(q_1)|
+ |\cro{\lag}_{i_1}(q_1)| - |\lag'(q_1)| \\
&+ \Bound! \times \left( \sum_{j=1}^m \cro{\nb{C_1 \cdots C_j}}_{i_1}(q) - \sum_{j=1}^m \nb{C_1 \cdots C_j}'(p)\right).
\end{aligned}
\end{equation*}


\subparagraph*{Previous operation: rest of Subsubsection~\ref{sssec:up-step}.}
Now let $\nb{\pi}'', \outi{\pi}''$, etc.
 denote the information of $\strans$ before applying Subsubsection~\ref{sssec:up-step}.
The operation builds $1 = i_1 < \cdots < i_{\ell} \le m$
and $\phi \defined B_1 \cdots B_{\ell}$ such that $B_j = \pre{a}{\Cf, C^x_{i}}(C_{i_j})$.
We first note that $C_{i_{\ell}} = S_0$ since $S_0, x[i], S_1$ is a step
and $\pre{C^x_i, C^x_{i+1}}{a}(C^x_{i+1}) = \Cf$.
Furthermore, we have $i_{\ell}  = m$ (otherwise $C^x_i \subseteq C_{i_{\ell}} \supsetneq C_{m} = S_1$
and $\pre{\Cf, C^x_{i_1}}{x[i_1]}(C_{m})  = \pre{C^x_{i_0}, C^x_{i_1}}{x[i_1]}(C_{m}) = S_0$).
Hence $\nb{\phi}'' = \nb{\rho}' \circ \pre{\Cf, C^x_{i_1}}{x[i]}$.
So  $\nb{\phi}''(q_0) = 0$ for $q_0 \defined \pre{\Cf, C^x_{i_1}}{x[i_1]}(q_1)  =  \pre{C^x_{i_0}, C^x_{i_2}}{x[i_1{:}i_2]}(q_2)$.


By definition 


By considering $\outi{C_1 \cdots C_{i_j}}'$
for $1 \le j \le n$, we see that $\outi{C_1 \cdots C_j}'' = \movi$ (if $j > 1$)
and $\nb{C_1 \cdots C_j}'' = \nb{D_1 \cdots D_{i_j}}'$ (which is $0$
when not in some $i_j$). Hence
$ \sum_{j=1}^n \nb{D_1 \cdots D_j}'(q) = \sum_{j=1}^m \nb{C_1 \cdots D_j}''(p)$.
Finally, we note that $c = \movi$ since there is no output,
and $|\val{S,\new{S}}{x[i{+}1{:}\new{i}]}(q)| = |\last'(q)| - |\last''(p)|
+|\lag'(q)| - |\lag''(p)|$.




If Subsubsection~\ref{sssec:prepro} was not used,
the proof is completed. Otherwise,
 let $\nb{\pi}''', \outi{\pi}'''$, etc.
 denote the information of $\strans$ right after Lemma~\ref{lem:sim:prune}).
Thanks to the above proof (and by a similar study of Algorithm~\ref{algo:down}),
we see that $\nb{\rho}'''(p) =0$, $\outi{C_1 C_2}''' = \cdots = \outi{C_1 \cdots C_n}'''= \movi$
and:
\begin{equation} 
\label{eq:labelle}
\begin{aligned}
|\val{S,\new{S}}{x[i{+}1{:}\new{i}]}(q)| = &|\new{\last(q)}| - |\last'''(p)|
+ |\new{\lag(q)}| - |\lag''''(p)| \\
&+ \Bound! \times \left( \sum_{j=1}^n \new{\nb{D_1 \cdots D_j}(q)} - \sum_{j=1}^m \nb{C_1 \cdots C_j}'''(p)\right)
\end{aligned}
\end{equation}
Let us finally consider the beginning of Subsubsection~\ref{sssec:prepro}.
Since there is no output, $c = \movi$ and $\lag(q) = \lag'''(q)$.
Let $\phi \defined C^x_i C_1 \cdots C_n \in \tree{C^x_i}$.
We had $\outi{C^x_i C_1} = \movi$ (by construction
and since there is no output) and $\outi{C^x_i C_1 \cdots C_j} = \outi{C_1 \cdots C_j}''' = \movi$
for all $j \ge 2$. Furthermore $\nb{\phi}(p) = \nb{\rho}'''(p) = \movi$.
Finally note that $|\last'''|(q) - |\last(p)| = \Bound! \nb{C^x_i}(q)$
and $\nb{C^x_i C_1 \cdots C_j}(p) = \nb{C_1 \cdots C_j}'''(p)$
for $j \ge 1$. This concludes the proof
by using Equation~\ref{eq:labelle}.


\subsection{Essai 3 : vieux}





\begin{sublemma} \label{lem:lazy} Let $N \le i \le \new{i}$.
Denote by $\nb{\pi}, \outi{\pi}$, etc. (resp.
$\new{\nb{\pi}}, \new{\outi{\pi}}$, etc.) the 
configuration of $\strans$ after reading $C^x_i$
(resp. $C^x_{\new{i}}$).
 Let $S \subseteq C^x_i$,
$\new{S} \subseteq C^x_{\new{i}}$ be such that $|S| = |\new{S}|$ and
$S, x[i{+}1{:}\new{i}], \new{S}$ is a step.
Assume that there exists
$\pi = D_1 \cdots D_{n} \in \tree{C^x_{\new{i}}}$
with $\new{S} = D_n$ and such that
$\new{\outi{D_1 D_2}} = \cdots = \new{\outi{D_1 \cdots D_n}} = \movi$.
Furthermore, let $q \in \new{S}$ be such that $\new{\nb{\pi}(q)} = 0$
\\
Let $p \defined \pre{S,\new{S}}{x[i{+}1{:}\new{i}]}(q)$,
then there exists $\rho = C_1 \cdots C_{m} \in \tree{C^x_{i}}$
with $C_m = S$, such that $\outi{C_1 C_2} = \cdots = \outi{C_1 \cdots C_m} = \movi$,
$\nb{\pi}(p) = 0$, and:
\begin{equation*} 
\begin{aligned}
|\val{S,\new{S}}{x[i{+}1{:}\new{i}]}(q)| = &|\new{\last(q)}| - |\last(p)|
+ |\new{\lag(q)}| - |\lag(p)| \\
&+ \Bound! \times \left( \sum_{j=1}^n \new{\nb{D_1 \cdots D_j}(q)} - \sum_{j=1}^m \nb{C_1 \cdots C_j}(p)\right)
\end{aligned}
\end{equation*}
\end{sublemma}

\begin{proof} By induction, it is enough to show the result for $\new{i} = i{+}1$.
Let us fix some $\pi$ and $q$ as in the statement of the lemma.
These values were obtained by possibly
applying Subsubsection~\ref{sssec:prepro}
(in the ``non-close'' case)
and then Subsubsection~\ref{sssec:up-step}.

We first consider the last operation of Subsubsection~\ref{sssec:up-step}, i.e. applying
Subsection~\ref{ssec:tool}. Let $\nb{\pi}', \outi{\pi}'$, etc.
be the information of $\strans$ before applying it.
Since Algorithm~\ref{algo:down}
cannot empty a register $\outi{D_1 \cdots D_j}$,
we necessarily had $\outi{D_1 D_2}' = \cdots = \outi{D_1 \cdots D_n}' = \movi$.
Since $\new{\nb{\pi}(q)} = 0$ and $\outi{\pi}' = \new{\outi{\pi}}$ remains unchanged,
we had $\nb{\pi}(q)' = 0$,
and furthermore $\nb{\pi\{q\}}'(q) = \new{\nb{\pi\{q\}}(q)}$.
By using the fact that Subsection~\ref{ssec:tool}
preserves invariant~\ref{inv:past}, we conclude
that:
\begin{equation*} 
\begin{aligned}
&|\new{\last(q)}| - |\last'(q)|
+ |\new{\lag(q)}| - |\lag'(q)| 
+ \Bound! \times \left( \sum_{j=1}^n \new{\nb{D_1 \cdots D_j}(q)} - \sum_{j=1}^n \nb{D_1 \cdots D_j}'(p)\right) = 0.
\end{aligned}
\end{equation*}


Now let $\nb''{\pi}, \outi''{\pi}$, etc.
 denote the information of $\strans$ before applying Subsubsection~\ref{sssec:up-step}.
The operation builds $1 = i_1 < \cdots < i_m \le n$
and $\rho \defined C_1 \cdots C_m$ such that $C_j = \pre{a}{\Cf, C^x_{i+1}}(D_{i_j})$.
We first note that $D_{i_m} = S$ since $S, a, \new{S}$ is a step
and $\pre{C^x_i, C^x_{i+1}}{a}(C^x_{i+1}) = \Cf$.
Since \gd{maximalité}, we must have $i_m = n$.
Hence $\nb{\rho}''(p) = 0$ if $p \defined \pre{\Cf, C^x_{i+1}}{a}(q)$.
By considering $\outi{C_1 \cdots C_{i_j}}'$
for $1 \le j \le n$, we see that $\outi{C_1 \cdots C_j}'' = \movi$ (if $j > 1$)
and $\nb{C_1 \cdots C_j}'' = \nb{D_1 \cdots D_{i_j}}'$ (which is $0$
when not in some $i_j$). Hence
$ \sum_{j=1}^n \nb{D_1 \cdots D_j}'(q) = \sum_{j=1}^m \nb{C_1 \cdots D_j}''(p)$.
Finally, we note that $c = \movi$ since there is no output,
and $|\val{S,\new{S}}{x[i{+}1{:}\new{i}]}(q)| = |\last'(q)| - |\last''(p)|
+|\lag'(q)| - |\lag''(p)|$.




If Subsubsection~\ref{sssec:prepro} was not used,
the proof is completed. Otherwise,
 let $\nb{\pi}''', \outi{\pi}'''$, etc.
 denote the information of $\strans$ right after Lemma~\ref{lem:sim:prune}).
Thanks to the above proof (and by a similar study of Algorithm~\ref{algo:down}),
we see that $\nb{\rho}'''(p) =0$, $\outi{C_1 C_2}''' = \cdots = \outi{C_1 \cdots C_n}'''= \movi$
and:
\begin{equation} 
\label{eq:labelle}
\begin{aligned}
|\val{S,\new{S}}{x[i{+}1{:}\new{i}]}(q)| = &|\new{\last(q)}| - |\last'''(p)|
+ |\new{\lag(q)}| - |\lag''''(p)| \\
&+ \Bound! \times \left( \sum_{j=1}^n \new{\nb{D_1 \cdots D_j}(q)} - \sum_{j=1}^m \nb{C_1 \cdots C_j}'''(p)\right)
\end{aligned}
\end{equation}
Let us finally consider the beginning of Subsubsection~\ref{sssec:prepro}.
Since there is no output, $c = \movi$ and $\lag(q) = \lag'''(q)$.
Let $\phi \defined C^x_i C_1 \cdots C_n \in \tree{C^x_i}$.
We had $\outi{C^x_i C_1} = \movi$ (by construction
and since there is no output) and $\outi{C^x_i C_1 \cdots C_j} = \outi{C_1 \cdots C_j}''' = \movi$
for all $j \ge 2$. Furthermore $\nb{\phi}(p) = \nb{\rho}'''(p) = \movi$.
Finally note that $|\last'''|(q) - |\last(p)| = \Bound! \nb{C^x_i}(q)$
and $\nb{C^x_i C_1 \cdots C_j}(p) = \nb{C_1 \cdots C_j}'''(p)$
for $j \ge 1$. This concludes the proof
by using Equation~\ref{eq:labelle}.
\end{proof}


\subsection{Proof of Lemma~\ref{lem:lazy}}

\gd{a-t-on vraiment besoin de prouver un résultat plus fort ?
l'expression exacte des prédécesseurs est horrible}




\begin{proof} By induction (and since a step can be decomposed
in some elementary steps),
it is sufficient to show the result with $i' = i{+}1$. Let $a \defined x[i{+}1]$.

First if $C^x_i, a, C^x_{i+1}$ is not a step, then $\strans$ applies
Subsubsection~\ref{sssec:prepro} and $C^x_i C' \in \tree{C^x_i}$
is not close. We first update $\out \leftarrow \out \outi{CC'}$.
But since $\strans$ is improductive from $i$ to $i{+}1$, we
necessarily had $\outi{C^x_i C'} = \movi$.
Thus $C' \neq S$ and since $S, a, S'$ is a
step with $S' \subseteq C^x_{i+1}$, we must have 
$C' \supsetneq S$. Now let $C_0 C_1 \cdots C_n \in \tree{C^x_i}$
be such that $C_0  = C^x_i$, $C_1 = C'$ and $C_n = S$,
there must exists $2 \le j \le n$ such that $\outi{C_0 C_1 \cdots C_j} \neq \movi$.
Since Algorithm~\ref{algo:down} cannot empty some $\outi{\pi}$, we conclude that
after applying Subsubsection~\ref{sssec:prepro} we have
$\Cf = C'$ and for all $C_1 \cdots C_n \in \tree{\Cf}$
with $C_n = S$, there exists $2 \le j \le n$ such that $\outi{C_1 \cdots C_j} \neq \movi$.

Let us show that Subsubsection~\ref{sssec:up-step} also preserves 
this property. Assume now that $\Cf, a,  C^x_{i+1}$ is a step.
Let $\pi = C_1 \cdots C_n \in \tree{C^x_{i+1}}$ be such that $C_n = S'$.
Following the notations of Subsubsection~\ref{sssec:up-step}, let
\gd{}
Finally, we apply Algorithm~\ref{algo:down}, which cannot empty some $\outi{\pi}$.
\end{proof}


\subsection{Subsets preserved infinitely}


%


\begin{sublemma} Assume that $\strans$ is $S^x_i$-prepared in $i \ge 0$.
Then there exists $i' \ge i$ such that  $\strans$ is 
not improductive (i.e. \emph{productive}) from $i$ to $i'$.
\end{sublemma}

\begin{proof} Assume the converse.

\end{proof}








